TaskMatrix.AI: Completing Tasks by Connecting Foundation Models with Millions of APIs

Artificial Intelligence (AI) has made incredible progress recently. On the one hand, advanced foundation models like ChatGPT can offer powerful conversation, in-context learning and code generation abilities on a broad range of open-domain tasks. They can also generate high-level solution outlines for domain-specific tasks based on the common sense knowledge they have acquired. However, they still face difficulties with some specialized tasks because they lack enough domain-specific data during pre-training or they often have errors in their neural network computations on those tasks that need accurate executions. On the other hand, there are also many existing models and systems (symbolic-based or neural-based) that can do some domain-specific tasks very well. However, due to the different implementation or working mechanisms, they are not easily accessible or compatible with foundation models. Therefore, there is a clear and pressing need for a mechanism that can leverage foundation models to propose task solution outlines and then automatically match some of the sub-tasks in the outlines to the off-the-shelf models and systems with special functionalities to complete them. Inspired by this, we introduce TaskMatrix.AI as a new AI ecosystem that connects foundation models with millions of APIs for task completion. Unlike most previous work that aimed to improve a single AI model, TaskMatrix.AI focuses more on using existing foundation models (as a brain-like central system) and APIs of other AI models and systems (as sub-task solvers) to achieve diversified tasks in both digital and physical domains. As a position paper, we will present our vision of how to build such an ecosystem, explain each key component, and use study cases to illustrate both the feasibility of this vision and the main challenges we need to address next.

==> case_study_codes/ppt_case2.tex <==
\newsavebox\lstboxnocomposition
\begin{lrbox}{\lstboxnocomposition}\begin{minipage}{0.98\linewidth}
MCFM: Sure, here's the code to generate slides for each company:
\begin{pythongray}
create_slide();
select_title();
insert_text("Microsoft");
select_content();
insert_text("Founded in 1975 by Bill Gates and Paul Allen in Albuquerque, New Mexico. The company's mission is to empower every person and every organization on the planet to achieve more. Some of its most popular products include Windows, Office, Xbox, and Surface. Microsoft has numerous subsidiaries, including LinkedIn, GitHub, and Minecraft.");
create_slide();
select_title();
insert_text("Apple");
select_content();
insert_text("Founded in 1976 by Steve Jobs, Steve Wozniak, and Ronald Wayne in Cupertino, California. Apple's mission is to design products and experiences that are easy to use and accessible to everyone. Some of its most popular products include the iPhone, iPad, MacBook, and Apple Watch. Apple has numerous subsidiaries, including Beats Electronics, Shazam, and Siri.");
...
\end{pythongray}
\end{minipage}\end{lrbox} 

\begin{tcolorbox}
...\\
\pyth{select_title()}: This API can be used to select the text box of the title. You should select the text box of context first and then insert or delete the text into the content.\\
\pyth{select_content()}: This API can be used to select the text box of content. You should select the text box of the title first and then insert or delete the text to the title.\\
...

Composition Instructions:\\
To generate a slide, you need to generate both the title and context.\\
\st{The context should contain several sentences, you can call insert\_text multiple times, or split the multiple sentences by '\textbackslash n'.}\\
...\\

\vspace{0.2cm}

\noindent\fcolorbox{white}{gray!15}{\usebox\lstboxnocomposition}
\end{tcolorbox}

% \refstepcounter{figure}
\captionof{figure}{After removing first type of composition instruction, MCFM generates a long paragraph for each slide. In contrast, when all composition instructions are included, MCFM generates several short sentences, as shown in Figure \ref{fig:ppt_case1}.}
\vspace{0.5cm}
\label{fig:ppt_case2}

